HEATS: Heterogeneity- and Energy-Aware Task-based Scheduling

Cloud providers usually offer diverse types of hardware for their users. Customers exploit this option to deploy cloud instances featuring GPUs, FPGAs, architectures other than x86 (e.g., ARM, IBM Power8), or featuring certain specific extensions (e.g, Intel SGX). We consider in this work the instances used by customers to deploy containers, nowadays the de facto standard for micro-services, or to execute computing tasks. In doing so, the underlying container orchestrator (e.g., Kubernetes) should be designed so as to take into account and exploit this hardware diversity. In addition, besides the feature range provided by different machines, there is an often overlooked diversity in the energy requirements introduced by hardware heterogeneity, which is simply ignored by default container orchestrator's placement strategies. We introduce HEATS, a new task-oriented and energy-aware orchestrator for containerized applications targeting heterogeneous clusters. HEATS allows customers to trade performance vs. energy requirements. Our system first learns the performance and energy features of the physical hosts. Then, it monitors the execution of tasks on the hosts and opportunistically migrates them onto different cluster nodes to match the customer-required deployment trade-offs. Our HEATS prototype is implemented within Google's Kubernetes. The evaluation with synthetic traces in our cluster indicate that our approach can yield considerable energy savings (up to 8.5%) and only marginally affect the overall runtime of deployed tasks (by at most 7%). HEATS is released as open-source.

==> traces.tex <==
\subsection{Traces}
\label{sec:traces}
\subsubsection{Google Borg Trace}
\subsubsection{Microsoft Azure Trace}
\subsubsection{OpenCloud Hadoop Cluster Trace}
\subsection{Trace Extraction and Sampling}
Recording of the Google Borg trace was started on May 1, 2011, at 19:00
EDT and lasted over a period of 29 days. It was made publicly available
after obfuscation~\cite{borg:obfuscation}. It contains datasets split
into several files that describe job as well as task events and usage
along with machine events and attributes~\cite{borg:techreport}. An
extract was chosen at random with a precise offset of 10 days from the
beginning of the trace.

Microsoft did record a trace of their Azure cloud computing service from
November 16, 2016 to February 16, 2017. A subset over a period of 30
days was made publicly available~\cite{azure:trace}, yet it does not
provide the same level of details as the Google Borg trace. For example,
the Azure trace is missing machine information, which would allow to
associate VMs to bare-metal machines running the VMs as well as their
attributes. An extract was taken right from the beginning of the trace.

Each of the two extracts comprise all recorded events over a duration of
12 hours. For both extracts a list of top 10 users was generated based on
the number of scheduled tasks in the Google Borg trace respectively the
number of scheduled VMs in the Microsoft Azure trace that were scheduled
during the 12 hours. Finally, a filter was applied to select only those
tasks respectively those VMs that were deployed by a top 10 user on the
previously generated list.

\subsubsection{Google Borg Trace Sampling}
The extracted Google Borg trace was further sampled, because the load of
the scheduled tasks of the top 10 users would exceed the resources of
the testbed. Since the Google Borg trace also includes machine
attributes, it is possible to apply a bijective mapping of a machine
type in the Google Borg trace to a machine type in the testbed with
matching machine attributes. Finally, because the sampled trace uses
more machines than are available on the testbed a surjective mapping of
several machines in the Google Borg trace to a single machine in the
testbed is applied. Machines of top 10 users in the trace are selected
according to the following properties: the machine was not added,
removed or updated during the 12 hour time frame; the machine has
scheduled at least one task; task usage for the machine is available.

\subsubsection{Microsoft Azure Trace Sampling}
\cg{complete this subsection if Azure trace needs to be sampled}
